WAX-ML: A Python library for machine learning and feedback loops on streaming data

Wax is what you put on a surfboard to avoid slipping. It is an essential tool to go surfing... We introduce WAX-ML a research-oriented Python library providing tools to design powerful machine learning algorithms and feedback loops working on streaming data. It strives to complement JAX with tools dedicated to time series. WAX-ML makes JAX-based programs easy to use for end-users working with pandas and xarray for data manipulation. It provides a simple mechanism for implementing feedback loops, allows the implementation of online learning and reinforcement learning algorithms with functions, and makes them easy to integrate by end-users working with the object-oriented reinforcement learning framework from the Gym library. It is released with an Apache open-source license on GitHub at https://github.com/eserie/wax-ml.

==> Makefile <==
# See https://stackoverflow.com/questions/38161093/makefile-converting-multiple-dot-files-to-png

BIB_FILES = $(wildcard *.bib)
TEX_FILES = $(wildcard *.tex)
TEX_PDF=$(TEX_FILES:.tex=.pdf)
TEX_PNG=$(TEX_FILES:.tex=.png)

.PHONY: all
all: pdf clean

%.pdf: %.tex
	latexmk -f -lualatex $<

.PHONY: pdf
pdf: $(TEX_PDF)

%.png: %.tex
	convert -density 300 -quality 90  $(<:.tex=.pdf)  $@

.PHONY: png
png: $(TEX_PNG)

clean:
	# see https://gist.github.com/djsutherland/266983
	latexmk -c
	rm -f *.dvi

.PHONY: clean-bib
clean-bib:
	bibtex-tidy \
	--curly \
	--numeric \
	--space=2 \
	--align=13 \
	--sort=key \
	--duplicates=key,doi,abstract,citation \
	--merge=combine \
	--strip-enclosing-braces \
	--drop-all-caps \
	--no-escape \
	--sort-fields=title,shorttitle,author,year,month,day,journal,booktitle,location,on,publisher,address,series,volume,number,pages,doi,isbn,issn,url,urldate,copyright,category,note,metadata \
	--trailing-commas \
	--encode-urls \
	--remove-empty-fields \
	--enclosing-braces=title \
	--wrap=88  wax-ml-paper.bib

